Efficient Determination of Safety Requirements for Perception Systems

Perception systems operate as a subcomponent of the general autonomy stack, and perception system designers often need to optimize performance characteristics while maintaining safety with respect to the overall closed-loop system. For this reason, it is useful to distill high-level safety requirements into component-level requirements on the perception system. In this work, we focus on efficiently determining sets of safe perception system performance characteristics given a black-box simulator of the fully-integrated, closed-loop system. We combine the advantages of common black-box estimation techniques such as Gaussian processes and threshold bandits to develop a new estimation method, which we call smoothing bandits. We demonstrate our method on a vision-based aircraft collision avoidance problem and show improvements in terms of both accuracy and efficiency over the Gaussian process and threshold bandit baselines.

==> figures/subplots/interp_points.tex <==
\addplot+[
  mark = {none},
  very thick, solid, cmap1
] coordinates {
  (0.0, 0.0)
  (0.01, 5.55302140759747e-8)
  (0.02, 1.9135669937070746e-5)
  (0.03, 0.0004931121316768381)
  (0.04, 0.004384042633961219)
  (0.05, 0.021712378626041674)
  (0.06, 0.07414882993501634)
  (0.07, 0.19564741410949074)
  (0.08, 0.4268663374621867)
  (0.09, 0.8045511202977738)
  (0.1, 1.3496296993122143)
  (0.11, 2.0582645019330164)
  (0.12, 2.898759511817386)
  (0.13, 3.81502845290161)
  (0.14, 4.735312861149776)
  (0.15, 5.583624353356332)
  (0.16, 6.291131437040081)
  (0.17, 6.80522758111631)
  (0.18, 7.094953399844824)
  (0.19, 7.152451198462425)
  (0.2, 6.990950258715774)
  (0.21, 6.640288849123563)
  (0.22, 6.141159692414489)
  (0.23, 5.539181099438977)
  (0.24, 4.879642809882539)
  (0.25, 4.203452157415147)
  (0.26, 3.5444916670129136)
  (0.27, 2.9283445900054517)
  (0.28, 2.372173234100139)
  (0.29, 1.8854470464098576)
  (0.3, 1.4711996450995195)
  (0.31, 1.1275259389503574)
  (0.32, 0.849090846101009)
  (0.33, 0.628491665258705)
  (0.34, 0.45738350469752215)
  (0.35, 0.32733320790639986)
  (0.36, 0.23040836954356478)
  (0.37, 0.15953416505221968)
  (0.38, 0.10866383254342409)
  (0.39, 0.07281180328525108)
  (0.4, 0.04799493914456515)
  (0.41, 0.0311200239787581)
  (0.42, 0.019846874385246547)
  (0.43, 0.012447789338393049)
  (0.44, 0.007676511414903049)
  (0.45, 0.004653870268267104)
  (0.46, 0.0027728978860127084)
  (0.47, 0.0016232910503859571)
  (0.48, 0.0009333795825527088)
  (0.49, 0.0005269365777112149)
  (0.5, 0.0002919557053360229)
  (0.51, 0.00015868484954802446)
  (0.52, 8.45658675881112e-5)
  (0.53, 4.416274343019859e-5)
  (0.54, 2.2586868968064067e-5)
  (0.55, 1.130600052049944e-5)
  (0.56, 5.534818507136171e-6)
  (0.57, 2.6478917536698304e-6)
  (0.58, 1.2368898509384297e-6)
  (0.59, 5.636315240062707e-7)
  (0.6, 2.5029816959850516e-7)
  (0.61, 1.0820440657169091e-7)
  (0.62, 4.5482280469420603e-8)
  (0.63, 1.8564743027972133e-8)
  (0.64, 7.348083016780058e-9)
  (0.65, 2.8159873392644318e-9)
  (0.66, 1.043109601473351e-9)
  (0.67, 3.7279805511496525e-10)
  (0.68, 1.2828802738106425e-10)
  (0.69, 4.241355100774276e-11)
  (0.7, 1.3439033998340796e-11)
  (0.71, 4.070088147020012e-12)
  (0.72, 1.1746607260302706e-12)
  (0.73, 3.219951288408753e-13)
  (0.74, 8.352236954973783e-14)
  (0.75, 2.0415897055162292e-14)
  (0.76, 4.680772307332727e-15)
  (0.77, 1.0012877194218144e-15)
  (0.78, 1.9865190526216455e-16)
  (0.79, 3.6303882646187706e-17)
  (0.8, 6.063682766590182e-18)
  (0.81, 9.173020530059594e-19)
  (0.82, 1.243681370420929e-19)
  (0.83, 1.4926827829649983e-20)
  (0.84, 1.5629664530165458e-21)
  (0.85, 1.4030921441237523e-22)
  (0.86, 1.0573924644785202e-23)
  (0.87, 6.519597311125541e-25)
  (0.88, 3.1854398121332274e-26)
  (0.89, 1.1846267614774096e-27)
  (0.9, 3.183752825412329e-29)
  (0.91, 5.7754676747589376e-31)
  (0.92, 6.446985556296304e-33)
  (0.93, 3.8897962739343996e-35)
  (0.94, 1.0490741982694744e-37)
  (0.95, 9.421051440833038e-41)
  (0.96, 1.7200359242788222e-44)
  (0.97, 2.531811107704389e-49)
  (0.98, 3.7667020685315644e-56)
  (0.99, 7.507122623395831e-68)
  (1.0, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap2
] coordinates {
  (1.1, 0.0)
  (1.11, 1.67930092957352e-15)
  (1.12, 1.9482219177601986e-11)
  (1.13, 4.012993378998176e-9)
  (1.14, 1.5834112053943477e-7)
  (1.15, 2.5218227169387535e-6)
  (1.16, 2.2594172483538378e-5)
  (1.17, 0.0001359329440829801)
  (1.18, 0.0006103484692524642)
  (1.19, 0.0021894467300756348)
  (1.2, 0.006573205848723772)
  (1.21, 0.017072209448652755)
  (1.22, 0.039307933245368305)
  (1.23, 0.08173224598364935)
  (1.24, 0.15569395605431474)
  (1.25, 0.2748229601462284)
  (1.26, 0.4536358778123458)
  (1.27, 0.705459282213059)
  (1.28, 1.0399631829437732)
  (1.29, 1.460740152709615)
  (1.3, 1.9634118557747875)
  (1.31, 2.5346800244679772)
  (1.32, 3.1525786860760197)
  (1.33, 3.7879677441417328)
  (1.34, 4.40708506793793)
  (1.35, 4.974792704819605)
  (1.36, 5.458046791288054)
  (1.37, 5.829104678253808)
  (1.38, 6.068051101832172)
  (1.39, 6.164356386509001)
  (1.4, 6.11734309177004)
  (1.41, 5.935601157021672)
  (1.42, 5.635528371792933)
  (1.43, 5.239264960625268)
  (1.44, 4.772331013000522)
  (1.45, 4.261266136590043)
  (1.46, 3.7315222734094147)
  (1.47, 3.2057874945247664)
  (1.48, 2.7028360798822457)
  (1.49, 2.2369217940122317)
  (1.5, 1.8176669208689145)
  (1.51, 1.450354951531454)
  (1.52, 1.136511301656639)
  (1.53, 0.8746521802520246)
  (1.54, 0.6610926079341382)
  (1.55, 0.4907254113390409)
  (1.56, 0.35770860662664605)
  (1.57, 0.2560244781482897)
  (1.58, 0.17989658489802834)
  (1.59, 0.12406892514695746)
  (1.6, 0.08396380671186393)
  (1.61, 0.05574181407724738)
  (1.62, 0.03628948405950424)
  (1.63, 0.023159077512244036)
  (1.64, 0.014481409240940504)
  (1.65, 0.008868190900419414)
  (1.66, 0.0053156366937135695)
  (1.67, 0.003116788847364695)
  (1.68, 0.0017864863221891307)
  (1.69, 0.0010002560883738446)
  (1.7, 0.0005466245371151779)
  (1.71, 0.00029130386115272)
  (1.72, 0.00015123692898956034)
  (1.73, 7.641141158616516e-5)
  (1.74, 3.752637152508888e-5)
  (1.75, 1.7890909257359045e-5)
  (1.76, 8.268565843615384e-6)
  (1.77, 3.698734053043802e-6)
  (1.78, 1.598659426487098e-6)
  (1.79, 6.66372049724666e-7)
  (1.8, 2.6731734111163146e-7)
  (1.81, 1.0296288969091253e-7)
  (1.82, 3.798043440724609e-8)
  (1.83, 1.3378885444939963e-8)
  (1.84, 4.486108977107636e-9)
  (1.85, 1.4267566137421158e-9)
  (1.86, 4.2865157341530956e-10)
  (1.87, 1.2110121184072123e-10)
  (1.88, 3.200571234806862e-11)
  (1.89, 7.866240333834888e-12)
  (1.9, 1.7857126802253157e-12)
  (1.91, 3.7148784538981204e-13)
  (1.92, 7.01763892550352e-14)
  (1.93, 1.190936298195157e-14)
  (1.94, 1.792756588492475e-15)
  (1.95, 2.35776045848961e-16)
  (1.96, 2.6598885657657193e-17)
  (1.97, 2.516954861977022e-18)
  (1.98, 1.9429055452134988e-19)
  (1.99, 1.1812540226707808e-20)
  (2.0, 5.406634909358309e-22)
  (2.01, 1.7553217150039397e-23)
  (2.02, 3.729246172226443e-25)
  (2.03, 4.630485752980063e-27)
  (2.04, 2.8475042143094536e-29)
  (2.05, 6.708764292656282e-32)
  (2.06, 3.9388448986616665e-35)
  (2.07, 2.5731129602965058e-39)
  (2.08, 3.059967573884485e-45)
  (2.09, 2.053168707074178e-55)
  (2.1, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap3
] coordinates {
  (2.2, 0.0)
  (2.21, 4.225635865982181e-24)
  (2.22, 1.6504316347618421e-18)
  (2.23, 2.7174124455677377e-15)
  (2.24, 4.758576111800299e-13)
  (2.25, 2.437171340536336e-11)
  (2.26, 5.72865856307063e-10)
  (2.27, 7.858500679418778e-9)
  (2.28, 7.26153061291249e-8)
  (2.29, 4.957691325873383e-7)
  (2.3, 2.6638158608266353e-6)
  (2.31, 1.1782640779313074e-5)
  (2.32, 4.435193723246533e-5)
  (2.33, 0.00014569795177315643)
  (2.34, 0.0004259505571711034)
  (2.35, 0.0011255225342298575)
  (2.36, 0.002721763545540905)
  (2.37, 0.006085070466296778)
  (2.38, 0.012683839644120872)
  (2.39, 0.024823064302974457)
  (2.4, 0.045882911377412995)
  (2.41, 0.08050515195517416)
  (2.42, 0.1346622418679891)
  (2.43, 0.21554171845836975)
  (2.44, 0.33119151010635406)
  (2.45, 0.48990089158717687)
  (2.46, 0.6993344302889419)
  (2.47, 0.9654857966804722)
  (2.48, 1.2915654494407596)
  (2.49, 1.6769707963877936)
  (2.5, 2.116500750474042)
  (2.51, 2.599963439212699)
  (2.52, 3.1122858862269136)
  (2.53, 3.634172709140502)
  (2.54, 4.143286655498593)
  (2.55, 4.6158492005845755)
  (2.56, 5.028496901153519)
  (2.57, 5.3601891848655985)
  (2.58, 5.59395228829621)
  (2.59, 5.7182636524123724)
  (2.6, 5.727927641476197)
  (2.61, 5.62435910773576)
  (2.62, 5.415265543632113)
  (2.63, 5.1137900902551205)
  (2.64, 4.737236459763651)
  (2.65, 4.3055355927367644)
  (2.66, 3.839629003290364)
  (2.67, 3.359935542635407)
  (2.68, 2.8850404211534117)
  (2.69, 2.430703879262393)
  (2.7, 2.0092391641225023)
  (2.71, 1.6292626190609851)
  (2.72, 1.295778708744182)
  (2.73, 1.0105337651781616)
  (2.74, 0.772556021926862)
  (2.75, 0.5787958740562817)
  (2.76, 0.4247873331629605)
  (2.77, 0.3052663235306464)
  (2.78, 0.21470033691739043)
  (2.79, 0.14770374019942206)
  (2.8, 0.09933102855038396)
  (2.81, 0.06525471476868923)
  (2.82, 0.04184444664404905)
  (2.83, 0.02616928544080282)
  (2.84, 0.015946429407830504)
  (2.85, 0.009457982129310743)
  (2.86, 0.005453744603223734)
  (2.87, 0.003053493040490139)
  (2.88, 0.001657639699972536)
  (2.89, 0.0008711506638701587)
  (2.9, 0.0004424361187650136)
  (2.91, 0.00021673147738966267)
  (2.92, 0.00010218138097168282)
  (2.93, 4.625459999935781e-5)
  (2.94, 2.0049391336610053e-5)
  (2.95, 8.296514616457085e-6)
  (2.96, 3.266297132952398e-6)
  (2.97, 1.218715822279194e-6)
  (2.98, 4.2906848976568273e-7)
  (2.99, 1.418226867305e-7)
  (3.0, 4.37573541425825e-8)
  (3.01, 1.2518180605949579e-8)
  (3.02, 3.2948623066410736e-9)
  (3.03, 7.90631114976164e-10)
  (3.04, 1.7110289547383274e-10)
  (3.05, 3.296685575731983e-11)
  (3.06, 5.5674334575669745e-12)
  (3.07, 8.085268436677058e-13)
  (3.08, 9.860486275530469e-14)
  (3.09, 9.800978185311552e-15)
  (3.1, 7.639749277479317e-16)
  (3.11, 4.439056314249749e-17)
  (3.12, 1.794939310547662e-18)
  (3.13, 4.586597285183509e-20)
  (3.14, 6.43112433821359e-22)
  (3.15, 3.975118255222563e-24)
  (3.16, 7.505240318965002e-27)
  (3.17, 2.1759592837568558e-30)
  (3.18, 2.0684105256592445e-35)
  (3.19, 4.672401170645659e-44)
  (3.2, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap4
] coordinates {
  (3.3000000000000003, 0.0)
  (3.31, 1.2414756280540848e-33)
  (3.3200000000000003, 1.6324475647805353e-26)
  (3.33, 2.148450061799846e-22)
  (3.3400000000000003, 1.6697171681296865e-19)
  (3.35, 2.7500472694510005e-17)
  (3.3600000000000003, 1.6958679141956023e-15)
  (3.37, 5.304412055816172e-14)
  (3.3800000000000003, 1.0086977960279973e-12)
  (3.39, 1.3107116816089977e-11)
  (3.4000000000000004, 1.2604155553412447e-10)
  (3.41, 9.49463187744388e-10)
  (3.4200000000000004, 5.842888040164875e-9)
  (3.43, 3.032466738494402e-8)
  (3.4400000000000004, 1.3605960754525935e-7)
  (3.45, 5.381928977261425e-7)
  (3.4600000000000004, 1.9066719480011077e-6)
  (3.47, 6.128325973445643e-6)
  (3.4800000000000004, 1.8062011210681595e-5)
  (3.49, 4.925160681588983e-5)
  (3.5000000000000004, 0.0001251910008797126)
  (3.5100000000000002, 0.0002985429310865924)
  (3.5200000000000005, 0.000671596357656143)
  (3.5300000000000002, 0.0014319867396319237)
  (3.54, 0.0029059594085447866)
  (3.5500000000000003, 0.005632796446602699)
  (3.5600000000000005, 0.010462010526254827)
  (3.5700000000000003, 0.018671212017057372)
  (3.58, 0.03209712949367053)
  (3.5900000000000003, 0.05326548020093598)
  (3.6, 0.08549812712656492)
  (3.6100000000000003, 0.13296959853533805)
  (3.62, 0.20068130311538607)
  (3.6300000000000003, 0.294322422692157)
  (3.64, 0.4199929397831865)
  (3.6500000000000004, 0.5837772301979512)
  (3.66, 0.7911756669740831)
  (3.6700000000000004, 1.0464249651303204)
  (3.68, 1.3517625009435914)
  (3.6900000000000004, 1.7067115860068791)
  (3.7, 2.1074793547421473)
  (3.7100000000000004, 2.546562670110687)
  (3.72, 3.012647663686259)
  (3.7300000000000004, 3.4908645491874544)
  (3.74, 3.963422875315563)
  (3.7500000000000004, 4.410607445685186)
  (3.7600000000000002, 4.81206764689923)
  (3.7700000000000005, 5.148289836699321)
  (3.7800000000000002, 5.402110607433883)
  (3.79, 5.560113728006462)
  (3.8000000000000003, 5.613758632960886)
  (3.8100000000000005, 5.560113728006462)
  (3.8200000000000003, 5.402110607433883)
  (3.83, 5.148289836699321)
  (3.8400000000000003, 4.81206764689923)
  (3.8500000000000005, 4.410607445685155)
  (3.8600000000000003, 3.963422875315563)
  (3.87, 3.4908645491874544)
  (3.8800000000000003, 3.012647663686259)
  (3.89, 2.546562670110687)
  (3.9000000000000004, 2.1074793547421473)
  (3.91, 1.7067115860068791)
  (3.9200000000000004, 1.3517625009435914)
  (3.93, 1.0464249651303204)
  (3.9400000000000004, 0.7911756669740831)
  (3.95, 0.5837772301979512)
  (3.9600000000000004, 0.4199929397831865)
  (3.97, 0.294322422692157)
  (3.9800000000000004, 0.20068130311538462)
  (3.99, 0.13296959853533805)
  (4.0, 0.08549812712656553)
  (4.01, 0.05326548020093598)
  (4.0200000000000005, 0.03209712949367053)
  (4.03, 0.018671212017057372)
  (4.04, 0.010462010526254827)
  (4.050000000000001, 0.005632796446602699)
  (4.0600000000000005, 0.0029059594085447866)
  (4.07, 0.0014319867396319237)
  (4.08, 0.0006715963576561382)
  (4.09, 0.00029854293108659026)
  (4.1000000000000005, 0.0001251910008797117)
  (4.11, 4.925160681589018e-5)
  (4.12, 1.8062011210681723e-5)
  (4.130000000000001, 6.128325973445686e-6)
  (4.140000000000001, 1.9066719480011212e-6)
  (4.15, 5.381928977261463e-7)
  (4.16, 1.3605960754525935e-7)
  (4.17, 3.032466738494402e-8)
  (4.180000000000001, 5.842888040164875e-9)
  (4.19, 9.494631877443745e-10)
  (4.2, 1.2604155553412356e-10)
  (4.21, 1.3107116816090069e-11)
  (4.220000000000001, 1.008697796027983e-12)
  (4.23, 5.304412055816021e-14)
  (4.24, 1.6958679141956507e-15)
  (4.25, 2.7500472694510787e-17)
  (4.26, 1.6697171681297104e-19)
  (4.2700000000000005, 2.1484500617998767e-22)
  (4.28, 1.6324475647805583e-26)
  (4.29, 1.2414756280540848e-33)
  (4.300000000000001, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap5
] coordinates {
  (4.4, 0.0)
  (4.41, 4.672401170645792e-44)
  (4.42, 2.0684105256592445e-35)
  (4.43, 2.1759592837568558e-30)
  (4.44, 7.505240318964895e-27)
  (4.45, 3.975118255222507e-24)
  (4.46, 6.431124338213499e-22)
  (4.47, 4.5865972851837047e-20)
  (4.48, 1.7949393105476877e-18)
  (4.49, 4.439056314249749e-17)
  (4.5, 7.639749277479425e-16)
  (4.51, 9.800978185311832e-15)
  (4.52, 9.86048627553054e-14)
  (4.53, 8.085268436677116e-13)
  (4.54, 5.567433457567013e-12)
  (4.55, 3.296685575731983e-11)
  (4.56, 1.7110289547383274e-10)
  (4.57, 7.90631114976164e-10)
  (4.58, 3.2948623066410736e-9)
  (4.59, 1.2518180605949756e-8)
  (4.6, 4.375735414258312e-8)
  (4.61, 1.41822686730502e-7)
  (4.62, 4.290684897656888e-7)
  (4.63, 1.2187158222792027e-6)
  (4.64, 3.266297132952398e-6)
  (4.65, 8.296514616457085e-6)
  (4.66, 2.0049391336610196e-5)
  (4.67, 4.6254599999358135e-5)
  (4.68, 0.00010218138097168282)
  (4.69, 0.00021673147738966112)
  (4.7, 0.0004424361187650136)
  (4.71, 0.0008711506638701525)
  (4.72, 0.0016576396999725478)
  (4.73, 0.0030534930404901824)
  (4.74, 0.005453744603223772)
  (4.75, 0.009457982129310809)
  (4.76, 0.015946429407830504)
  (4.77, 0.02616928544080282)
  (4.78, 0.04184444664404934)
  (4.79, 0.06525471476868923)
  (4.8, 0.09933102855038467)
  (4.81, 0.14770374019942206)
  (4.82, 0.21470033691739196)
  (4.83, 0.3052663235306464)
  (4.84, 0.4247873331629635)
  (4.85, 0.5787958740562859)
  (4.86, 0.772556021926862)
  (4.87, 1.0105337651781616)
  (4.88, 1.295778708744182)
  (4.89, 1.6292626190609851)
  (4.9, 2.0092391641225023)
  (4.91, 2.430703879262393)
  (4.92, 2.8850404211534117)
  (4.93, 3.359935542635431)
  (4.94, 3.839629003290364)
  (4.95, 4.3055355927367644)
  (4.96, 4.737236459763651)
  (4.97, 5.113790090255157)
  (4.98, 5.415265543632113)
  (4.99, 5.6243591077358)
  (5.0, 5.727927641476197)
  (5.01, 5.7182636524123724)
  (5.02, 5.59395228829621)
  (5.03, 5.3601891848655985)
  (5.04, 5.028496901153519)
  (5.05, 4.6158492005845755)
  (5.06, 4.143286655498593)
  (5.07, 3.634172709140502)
  (5.08, 3.1122858862269136)
  (5.09, 2.5999634392127176)
  (5.1, 2.116500750474042)
  (5.11, 1.6769707963877936)
  (5.12, 1.2915654494407596)
  (5.13, 0.9654857966804722)
  (5.14, 0.6993344302889419)
  (5.15, 0.48990089158717687)
  (5.16, 0.33119151010635406)
  (5.17, 0.21554171845836975)
  (5.18, 0.13466224186798817)
  (5.19, 0.08050515195517416)
  (5.2, 0.04588291137741267)
  (5.21, 0.024823064302974457)
  (5.22, 0.012683839644120872)
  (5.23, 0.006085070466296778)
  (5.24, 0.002721763545540905)
  (5.25, 0.0011255225342298575)
  (5.26, 0.0004259505571711034)
  (5.27, 0.00014569795177315643)
  (5.28, 4.435193723246565e-5)
  (5.29, 1.178264077931299e-5)
  (5.3, 2.6638158608266162e-6)
  (5.31, 4.957691325873383e-7)
  (5.32, 7.261530612912386e-8)
  (5.33, 7.858500679418665e-9)
  (5.34, 5.728658563070712e-10)
  (5.35, 2.4371713405363707e-11)
  (5.36, 4.758576111800366e-13)
  (5.37, 2.7174124455677764e-15)
  (5.38, 1.6504316347618655e-18)
  (5.39, 4.225635865982181e-24)
  (5.4, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap6
] coordinates {
  (5.5, 0.0)
  (5.51, 2.053168707074178e-55)
  (5.52, 3.059967573884399e-45)
  (5.53, 2.5731129602964327e-39)
  (5.54, 3.938844898661554e-35)
  (5.55, 6.708764292656091e-32)
  (5.56, 2.8475042143092916e-29)
  (5.57, 4.630485752980195e-27)
  (5.58, 3.729246172226496e-25)
  (5.59, 1.7553217150039397e-23)
  (5.6, 5.406634909358386e-22)
  (5.61, 1.1812540226707977e-20)
  (5.62, 1.9429055452134988e-19)
  (5.63, 2.516954861977022e-18)
  (5.64, 2.6598885657657193e-17)
  (5.65, 2.3577604584895764e-16)
  (5.66, 1.7927565884924495e-15)
  (5.67, 1.1909362981951487e-14)
  (5.68, 7.017638925503469e-14)
  (5.69, 3.714878453898147e-13)
  (5.7, 1.7857126802253282e-12)
  (5.71, 7.866240333834944e-12)
  (5.72, 3.2005712348068846e-11)
  (5.73, 1.2110121184072123e-10)
  (5.74, 4.2865157341530956e-10)
  (5.75, 1.4267566137421158e-9)
  (5.76, 4.486108977107636e-9)
  (5.77, 1.3378885444939963e-8)
  (5.78, 3.798043440724609e-8)
  (5.79, 1.029628896909118e-7)
  (5.8, 2.6731734111162955e-7)
  (5.81, 6.663720497246613e-7)
  (5.82, 1.5986594264871094e-6)
  (5.83, 3.6987340530438285e-6)
  (5.84, 8.268565843615384e-6)
  (5.85, 1.7890909257359045e-5)
  (5.86, 3.752637152508888e-5)
  (5.87, 7.641141158616516e-5)
  (5.88, 0.00015123692898956034)
  (5.89, 0.00029130386115272)
  (5.9, 0.0005466245371151779)
  (5.91, 0.0010002560883738375)
  (5.92, 0.0017864863221891307)
  (5.93, 0.003116788847364695)
  (5.94, 0.0053156366937135695)
  (5.95, 0.008868190900419414)
  (5.96, 0.014481409240940504)
  (5.97, 0.023159077512244036)
  (5.98, 0.03628948405950424)
  (5.99, 0.05574181407724738)
  (6.0, 0.08396380671186393)
  (6.01, 0.12406892514695746)
  (6.02, 0.17989658489802834)
  (6.03, 0.2560244781482897)
  (6.04, 0.35770860662664605)
  (6.05, 0.4907254113390427)
  (6.06, 0.6610926079341382)
  (6.07, 0.8746521802520215)
  (6.08, 1.136511301656635)
  (6.09, 1.450354951531454)
  (6.1, 1.8176669208689145)
  (6.11, 2.2369217940122317)
  (6.12, 2.7028360798822457)
  (6.13, 3.2057874945247664)
  (6.14, 3.7315222734094147)
  (6.15, 4.261266136590043)
  (6.16, 4.772331013000522)
  (6.17, 5.239264960625268)
  (6.18, 5.635528371792913)
  (6.19, 5.935601157021672)
  (6.2, 6.11734309177004)
  (6.21, 6.164356386509001)
  (6.22, 6.068051101832172)
  (6.23, 5.829104678253808)
  (6.24, 5.458046791288054)
  (6.25, 4.974792704819605)
  (6.26, 4.40708506793793)
  (6.27, 3.7879677441417328)
  (6.28, 3.1525786860760197)
  (6.29, 2.5346800244679772)
  (6.3, 1.9634118557747875)
  (6.31, 1.460740152709615)
  (6.32, 1.0399631829437732)
  (6.33, 0.7054592822130615)
  (6.34, 0.4536358778123458)
  (6.35, 0.2748229601462284)
  (6.36, 0.15569395605431474)
  (6.37, 0.08173224598364935)
  (6.38, 0.039307933245368305)
  (6.39, 0.017072209448652634)
  (6.4, 0.006573205848723725)
  (6.41, 0.0021894467300756504)
  (6.42, 0.0006103484692524598)
  (6.43, 0.00013593294408297817)
  (6.44, 2.25941724835387e-5)
  (6.45, 2.5218227169387717e-6)
  (6.46, 1.5834112053943702e-7)
  (6.47, 4.012993378998176e-9)
  (6.48, 1.9482219177602264e-11)
  (6.49, 1.67930092957352e-15)
  (6.5, 0.0)
};

\addplot+[
  mark = {none},
  very thick, solid, cmap7
] coordinates {
  (6.6, 0.0)
  (6.61, 7.507122623395831e-68)
  (6.62, 3.76670206853135e-56)
  (6.63, 2.5318111077043173e-49)
  (6.64, 1.7200359242787731e-44)
  (6.65, 9.421051440832503e-41)
  (6.66, 1.0490741982694445e-37)
  (6.67, 3.88979627393451e-35)
  (6.68, 6.446985556296304e-33)
  (6.69, 5.7754676747589376e-31)
  (6.7, 3.183752825412329e-29)
  (6.71, 1.1846267614774265e-27)
  (6.72, 3.1854398121332274e-26)
  (6.73, 6.519597311125541e-25)
  (6.74, 1.0573924644785202e-23)
  (6.75, 1.4030921441237323e-22)
  (6.76, 1.5629664530165458e-21)
  (6.77, 1.492682782964977e-20)
  (6.78, 1.243681370420929e-19)
  (6.79, 9.173020530059725e-19)
  (6.8, 6.063682766590182e-18)
  (6.81, 3.6303882646188224e-17)
  (6.82, 1.9865190526216595e-16)
  (6.83, 1.0012877194218144e-15)
  (6.84, 4.680772307332727e-15)
  (6.85, 2.0415897055162292e-14)
  (6.86, 8.352236954973783e-14)
  (6.87, 3.219951288408753e-13)
  (6.88, 1.1746607260302706e-12)
  (6.89, 4.070088147019983e-12)
  (6.9, 1.34390339983407e-11)
  (6.91, 4.241355100774246e-11)
  (6.92, 1.2828802738106516e-10)
  (6.93, 3.727980551149705e-10)
  (6.94, 1.0431096014733584e-9)
  (6.95, 2.8159873392644318e-9)
  (6.96, 7.348083016780058e-9)
  (6.97, 1.8564743027972133e-8)
  (6.98, 4.5482280469420603e-8)
  (6.99, 1.0820440657169091e-7)
  (7.0, 2.5029816959850516e-7)
  (7.01, 5.636315240062707e-7)
  (7.02, 1.2368898509384208e-6)
  (7.03, 2.6478917536698304e-6)
  (7.04, 5.53481850713621e-6)
  (7.05, 1.130600052049944e-5)
  (7.06, 2.2586868968064226e-5)
  (7.07, 4.416274343019859e-5)
  (7.08, 8.45658675881112e-5)
  (7.09, 0.00015868484954802446)
  (7.1, 0.0002919557053360229)
  (7.11, 0.0005269365777112149)
  (7.12, 0.0009333795825527088)
  (7.13, 0.0016232910503859571)
  (7.14, 0.0027728978860127283)
  (7.15, 0.00465387026826712)
  (7.16, 0.007676511414903077)
  (7.17, 0.012447789338393005)
  (7.18, 0.019846874385246405)
  (7.19, 0.031120023978757877)
  (7.2, 0.04799493914456515)
  (7.21, 0.07281180328525108)
  (7.22, 0.10866383254342409)
  (7.23, 0.15953416505221968)
  (7.24, 0.23040836954356478)
  (7.25, 0.32733320790639986)
  (7.26, 0.45738350469752054)
  (7.27, 0.6284916652587074)
  (7.28, 0.849090846101009)
  (7.29, 1.1275259389503534)
  (7.3, 1.4711996450995142)
  (7.31, 1.8854470464098576)
  (7.32, 2.372173234100139)
  (7.33, 2.9283445900054517)
  (7.34, 3.5444916670129136)
  (7.35, 4.203452157415147)
  (7.36, 4.879642809882539)
  (7.37, 5.539181099438977)
  (7.38, 6.141159692414489)
  (7.39, 6.640288849123563)
  (7.4, 6.990950258715774)
  (7.41, 7.15245119846245)
  (7.42, 7.094953399844799)
  (7.43, 6.80522758111631)
  (7.44, 6.291131437040081)
  (7.45, 5.583624353356332)
  (7.46, 4.735312861149776)
  (7.47, 3.81502845290161)
  (7.48, 2.898759511817386)
  (7.49, 2.0582645019330092)
  (7.5, 1.3496296993122094)
  (7.51, 0.8045511202977738)
  (7.52, 0.4268663374621867)
  (7.53, 0.19564741410949005)
  (7.54, 0.0741488299350166)
  (7.55, 0.021712378626041827)
  (7.56, 0.0043840426339612345)
  (7.57, 0.0004931121316768417)
  (7.58, 1.9135669937070885e-5)
  (7.59, 5.553021407597431e-8)
  (7.6, 0.0)
};

==> figures/subplots/kernel_points_1.tex <==
\addplot+[
  mark = {none},
  very thick, solid, cmap1
] coordinates {
  (0.0, 0.0)
  (0.01, 5.553021267064501e-8)
  (0.02, 1.9135669567948048e-5)
  (0.03, 0.0004931121238963611)
  (0.04, 0.004384042575683702)
  (0.05, 0.021712378379165256)
  (0.06, 0.07414882920810933)
  (0.07, 0.1956474124500064)
  (0.08, 0.4268663343287608)
  (0.09, 0.8045511151997532)
  (0.1, 1.3496296919690438)
  (0.11, 2.058264492396913)
  (0.12, 2.898759500518541)
  (0.13, 3.8150284406037382)
  (0.14, 4.735312848832241)
  (0.15, 5.58362434205671)
  (0.16, 6.291131427695903)
  (0.17, 6.805227574438615)
  (0.18, 7.094953396242637)
  (0.19, 7.152451198023355)
  (0.2, 6.990950261235745)
  (0.21, 6.640288854171504)
  (0.22, 6.141159699414375)
  (0.23, 5.539181107753939)
  (0.24, 4.879642818888335)
  (0.25, 4.203452166555833)
  (0.26, 3.544491675836007)
  (0.27, 2.928344598177435)
  (0.28, 2.3721732414057843)
  (0.29, 1.8854470527398628)
  (0.3, 1.471199650431297)
  (0.31, 1.1275259433260758)
  (0.32, 0.849090849606087)
  (0.33, 0.6284916680028946)
  (0.34, 0.4573835067997169)
  (0.35, 0.32733320948347794)
  (0.36, 0.23040837070302383)
  (0.37, 0.1595341658880524)
  (0.38, 0.10866383313448551)
  (0.39, 0.07281180369539621)
  (0.4, 0.04799493942390843)
  (0.41, 0.031120024165527345)
  (0.42, 0.019846874507843303)
  (0.43, 0.01244778941740104)
  (0.44, 0.0076765114648912084)
  (0.45, 0.004653870299314832)
  (0.46, 0.0027728979049403794)
  (0.47, 0.0016232910617095773)
  (0.48, 0.0009333795891991413)
  (0.49, 0.0005269365815375153)
  (0.5, 0.00029195570749579106)
  (0.51, 0.00015868485074283875)
  (0.52, 8.456586823564771e-5)
  (0.53, 4.416274377381999e-5)
  (0.54, 2.2586869146509294e-5)
  (0.55, 1.1306000611128847e-5)
  (0.56, 5.534818552122298e-6)
  (0.57, 2.647891775477341e-6)
  (0.58, 1.2368898612540941e-6)
  (0.59, 5.636315287635875e-7)
  (0.6, 2.50298171735363e-7)
  (0.61, 1.0820440750553221e-7)
  (0.62, 4.548228086601546e-8)
  (0.63, 1.856474319144491e-8)
  (0.64, 7.348083082087169e-9)
  (0.65, 2.815987364512808e-9)
  (0.66, 1.0431096109038928e-9)
  (0.67, 3.727980585118243e-10)
  (0.68, 1.2828802855861696e-10)
  (0.69, 4.241355139974271e-11)
  (0.7, 1.3439034123347432e-11)
  (0.71, 4.070088185104501e-12)
  (0.72, 1.174660737082019e-12)
  (0.73, 3.2199513188550413e-13)
  (0.74, 8.352237034304714e-14)
  (0.75, 2.0415897249853264e-14)
  (0.76, 4.680772352125698e-15)
  (0.77, 1.0012877290320574e-15)
  (0.78, 1.986519071733813e-16)
  (0.79, 3.630388299609874e-17)
  (0.8, 6.063682825103956e-18)
  (0.81, 9.173020618624883e-19)
  (0.82, 1.2436813824263977e-19)
  (0.83, 1.492682797360226e-20)
  (0.84, 1.5629664680621934e-21)
  (0.85, 1.4030921575929693e-22)
  (0.86, 1.0573924745902021e-23)
  (0.87, 6.5195973731569055e-25)
  (0.88, 3.185439842245949e-26)
  (0.89, 1.1846267725853817e-27)
  (0.9, 3.183752854965521e-29)
  (0.91, 5.775467727702381e-31)
  (0.92, 6.446985614482739e-33)
  (0.93, 3.889796308363387e-35)
  (0.94, 1.0490742073276172e-37)
  (0.95, 9.42105151959347e-41)
  (0.96, 1.720035938043804e-44)
  (0.97, 2.5318111267300463e-49)
  (0.98, 3.7667020941033084e-56)
  (0.99, 7.507122664564657e-68)
  (1.0, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap2
] coordinates {
  (1.1, 0.0)
  (1.11, 0.00022385869436292264)
  (1.12, 0.005231457292727772)
  (1.13, 0.03018443568542441)
  (1.14, 0.09809423641441246)
  (1.15, 0.23251028728581488)
  (1.16, 0.450983932417571)
  (1.17, 0.7611173432291509)
  (1.18, 1.159345608845541)
  (1.19, 1.6318925357645344)
  (1.2, 2.1571270378478182)
  (1.21, 2.7085831932496465)
  (1.22, 3.2580541224949537)
  (1.23, 3.778349257077211)
  (1.24, 4.245474323222538)
  (1.25, 4.640133720081456)
  (1.26, 4.948559440389315)
  (1.27, 5.162740268782053)
  (1.28, 5.280164514162808)
  (1.29, 5.303205320275864)
  (1.3, 5.238276130501398)
  (1.31, 5.094871021952669)
  (1.32, 4.8845852583143285)
  (1.33, 4.620189344576236)
  (1.34, 4.314807861474385)
  (1.35, 3.9812342555973284)
  (1.36, 3.6313956462303505)
  (1.37, 3.2759680739859776)
  (1.38, 2.924132516908978)
  (1.39, 2.5834551987738554)
  (1.4, 2.259871791719743)
  (1.41, 1.9577535595747861)
  (1.42, 1.6800337632728721)
  (1.43, 1.4283742426462325)
  (1.44, 1.2033545399134054)
  (1.45, 1.0046688499788141)
  (1.46, 0.8313191587484179)
  (1.47, 0.6817959266782201)
  (1.48, 0.5542404245847597)
  (1.49, 0.44658522754979973)
  (1.5, 0.35667136661700277)
  (1.51, 0.2823422130768622)
  (1.52, 0.2215153424293247)
  (1.53, 0.1722344310657375)
  (1.54, 0.13270372732010965)
  (1.55, 0.10130786482105444)
  (1.56, 0.07661980600216864)
  (1.57, 0.0573995704217351)
  (1.58, 0.042586164172310946)
  (1.59, 0.03128482436497668)
  (1.6, 0.02275136030360772)
  (1.61, 0.016375036968185618)
  (1.62, 0.011661126284278263)
  (1.63, 0.008213960628469267)
  (1.64, 0.005721069063235283)
  (1.65, 0.0039387635495426185)
  (1.66, 0.0026793701511930402)
  (1.67, 0.0018001668904647687)
  (1.68, 0.0011939916817980778)
  (1.69, 0.0007814159534198435)
  (1.7, 0.0005043370595420604)
  (1.71, 0.000320820299023959)
  (1.72, 0.00020101451725319382)
  (1.73, 0.00012396961440444632)
  (1.74, 7.519617150968512e-5)
  (1.75, 4.482384901129432e-5)
  (1.76, 2.623386687190832e-5)
  (1.77, 1.5059990300662318e-5)
  (1.78, 8.470790810785883e-6)
  (1.79, 4.662735449906326e-6)
  (1.8, 2.5084345795712574e-6)
  (1.81, 1.3169748340411654e-6)
  (1.82, 6.736959264592132e-7)
  (1.83, 3.351836751690466e-7)
  (1.84, 1.6186948914353487e-7)
  (1.85, 7.57071634795969e-8)
  (1.86, 3.420617099533488e-8)
  (1.87, 1.4887838273977608e-8)
  (1.88, 6.2218012488453185e-9)
  (1.89, 2.4874712303718774e-9)
  (1.9, 9.4737430358482e-10)
  (1.91, 3.420476114028617e-10)
  (1.92, 1.1640911316490917e-10)
  (1.93, 3.709642367306888e-11)
  (1.94, 1.0982546265627384e-11)
  (1.95, 2.992381905051012e-12)
  (1.96, 7.418964550320433e-13)
  (1.97, 1.6506381010851057e-13)
  (1.98, 3.239372502992408e-14)
  (1.99, 5.486942836052174e-15)
  (2.0, 7.800352114403482e-16)
  (2.01, 8.970480802249544e-17)
  (2.02, 7.93903835915561e-18)
  (2.03, 5.041859218374425e-19)
  (2.04, 2.0738993023824888e-20)
  (2.05, 4.71379859681754e-22)
  (2.06, 4.536934951263652e-24)
  (2.07, 1.1227627487467236e-26)
  (2.08, 2.330768419749855e-30)
  (2.09, 1.1380666180635539e-36)
  (2.1, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap3
] coordinates {
  (2.2, 0.0)
  (2.21, 0.47066834850941996)
  (2.22, 0.7728939767077169)
  (2.23, 1.0184311582518466)
  (2.24, 1.2260672978458833)
  (2.25, 1.4045250049732725)
  (2.26, 1.5589862316946708)
  (2.27, 1.6929594833989912)
  (2.28, 1.8090234634828075)
  (2.29, 1.9091831031739843)
  (2.3, 1.9950618979636288)
  (2.31, 2.0680151815294257)
  (2.32, 2.129201328879502)
  (2.33, 2.1796288612206487)
  (2.34, 2.220188921015306)
  (2.35, 2.251678436604755)
  (2.36, 2.274817125543972)
  (2.37, 2.2902602840658974)
  (2.38, 2.2986086122139873)
  (2.39, 2.3004159021845565)
  (2.4, 2.296195153211241)
  (2.41, 2.2864235058195064)
  (2.42, 2.2715462752790025)
  (2.43, 2.251980287405376)
  (2.44, 2.2281166667280696)
  (2.45, 2.2003231895165936)
  (2.46, 2.1689462872017766)
  (2.47, 2.1343127660618064)
  (2.48, 2.0967312944898215)
  (2.49, 2.0564936982505735)
  (2.5, 2.0138760958577024)
  (2.51, 1.9691398998556766)
  (2.52, 1.9225327048721397)
  (2.53, 1.8742890794594573)
  (2.54, 1.8246312757086864)
  (2.55, 1.773769868204152)
  (2.56, 1.721904331950768)
  (2.57, 1.6692235673428188)
  (2.58, 1.615906378972136)
  (2.59, 1.5621219140338474)
  (2.6, 1.5080300652322693)
  (2.61, 1.4537818423813669)
  (2.62, 1.3995197163050244)
  (2.63, 1.345377938149723)
  (2.64, 1.29148283680831)
  (2.65, 1.2379530968042751)
  (2.66, 1.1849000186899605)
  (2.67, 1.1324277637603022)
  (2.68, 1.0806335846686703)
  (2.69, 1.0296080433470993)
  (2.7, 0.9794352174747972)
  (2.71, 0.9301928966022275)
  (2.72, 0.8819527689199951)
  (2.73, 0.8347805995594151)
  (2.74, 0.7887364012227938)
  (2.75, 0.7438745978641114)
  (2.76, 0.7002441820734954)
  (2.77, 0.6578888667601318)
  (2.78, 0.6168472316771018)
  (2.79, 0.5771528652870347)
  (2.8, 0.5388345024286488)
  (2.81, 0.5019161582106187)
  (2.82, 0.4664172585301353)
  (2.83, 0.43235276758860663)
  (2.84, 0.3997333127557974)
  (2.85, 0.36856530711605007)
  (2.86, 0.3388510700158006)
  (2.87, 0.3105889459202833)
  (2.88, 0.28377342187898597)
  (2.89, 0.25839524389400687)
  (2.9, 0.2344415324830664)
  (2.91, 0.21189589772955342)
  (2.92, 0.1907385541158631)
  (2.93, 0.17094643544365187)
  (2.94, 0.15249331015584094)
  (2.95, 0.13534989739075926)
  (2.96, 0.11948398411935818)
  (2.97, 0.10486054374282056)
  (2.98, 0.09144185656123288)
  (2.99, 0.0791876325657462)
  (3.0, 0.06805513705875486)
  (3.01, 0.057999319671589576)
  (3.02, 0.04897294743046157)
  (3.03, 0.04092674262348671)
  (3.04, 0.033809526350838684)
  (3.05, 0.027568368805149308)
  (3.06, 0.02214874754251326)
  (3.07, 0.017494715283614435)
  (3.08, 0.01354907915569475)
  (3.09, 0.010253593788755273)
  (3.1, 0.0075491713746771985)
  (3.11, 0.005376112783936046)
  (3.12, 0.0036743652745334903)
  (3.13, 0.002383814506011359)
  (3.14, 0.0014446220105188865)
  (3.15, 0.0007976249991031814)
  (3.16, 0.0003848255861026061)
  (3.17, 0.000150016422386454)
  (3.18, 3.9633866479958847e-5)
  (3.19, 4.049452898020793e-6)
  (3.2, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap4
] coordinates {
  (3.3000000000000003, 0.0)
  (3.31, 0.6089267467622664)
  (3.3200000000000003, 0.6912056133474113)
  (3.33, 0.7438012742282117)
  (3.3400000000000003, 0.7830796513890238)
  (3.35, 0.8146012794390541)
  (3.3600000000000003, 0.840979642438625)
  (3.37, 0.8636673070291221)
  (3.3800000000000003, 0.8835608439179528)
  (3.39, 0.9012551684123198)
  (3.4000000000000004, 0.917166573219289)
  (3.41, 0.9315984701395528)
  (3.4200000000000004, 0.9447792449079065)
  (3.43, 0.9568853653593689)
  (3.4400000000000004, 0.968056166258551)
  (3.45, 0.9784036817728774)
  (3.4600000000000004, 0.9880193998628378)
  (3.47, 0.9969790319134442)
  (3.4800000000000004, 1.0053459617748695)
  (3.49, 1.0131737919491977)
  (3.5000000000000004, 1.020508257704916)
  (3.5100000000000002, 1.0273886893389081)
  (3.5200000000000005, 1.0338491453627772)
  (3.5300000000000002, 1.0399193020115338)
  (3.54, 1.045625159589076)
  (3.5500000000000003, 1.0509896092569178)
  (3.5600000000000005, 1.0560328921696316)
  (3.5700000000000003, 1.0607729746230141)
  (3.58, 1.0652258569934157)
  (3.5900000000000003, 1.0694058299791678)
  (3.6, 1.073325688521657)
  (3.6100000000000003, 1.0769969114553064)
  (3.62, 1.0804298131864751)
  (3.6300000000000003, 1.0836336723734472)
  (3.64, 1.0866168415619961)
  (3.6500000000000004, 1.089386840943961)
  (3.66, 1.0919504387923693)
  (3.6700000000000004, 1.0943137206438789)
  (3.68, 1.0964821489167567)
  (3.6900000000000004, 1.09846061434713)
  (3.7, 1.1002534803805368)
  (3.7100000000000004, 1.1018646214567112)
  (3.72, 1.1032974559630007)
  (3.7300000000000004, 1.104554974498112)
  (3.74, 1.1056397639769802)
  (3.7500000000000004, 1.1065540280147264)
  (3.7600000000000002, 1.1072996039492322)
  (3.7700000000000005, 1.107877976794744)
  (3.7800000000000002, 1.1082902903608172)
  (3.79, 1.108537355719742)
  (3.8000000000000003, 1.108619657159795)
  (3.8100000000000005, 1.108537355719742)
  (3.8200000000000003, 1.1082902903608172)
  (3.83, 1.107877976794744)
  (3.8400000000000003, 1.107299603949232)
  (3.8500000000000005, 1.1065540280147264)
  (3.8600000000000003, 1.1056397639769802)
  (3.87, 1.104554974498112)
  (3.8800000000000003, 1.1032974559630007)
  (3.89, 1.1018646214567112)
  (3.9000000000000004, 1.1002534803805368)
  (3.91, 1.09846061434713)
  (3.9200000000000004, 1.0964821489167567)
  (3.93, 1.0943137206438789)
  (3.9400000000000004, 1.0919504387923693)
  (3.95, 1.089386840943961)
  (3.9600000000000004, 1.0866168415619961)
  (3.97, 1.0836336723734472)
  (3.9800000000000004, 1.0804298131864751)
  (3.99, 1.0769969114553064)
  (4.0, 1.073325688521657)
  (4.01, 1.0694058299791678)
  (4.0200000000000005, 1.0652258569934157)
  (4.03, 1.0607729746230141)
  (4.04, 1.0560328921696316)
  (4.050000000000001, 1.0509896092569178)
  (4.0600000000000005, 1.045625159589076)
  (4.07, 1.0399193020115338)
  (4.08, 1.0338491453627772)
  (4.09, 1.0273886893389081)
  (4.1000000000000005, 1.020508257704916)
  (4.11, 1.0131737919491977)
  (4.12, 1.0053459617748695)
  (4.130000000000001, 0.9969790319134443)
  (4.140000000000001, 0.9880193998628378)
  (4.15, 0.9784036817728774)
  (4.16, 0.968056166258551)
  (4.17, 0.9568853653593689)
  (4.180000000000001, 0.9447792449079065)
  (4.19, 0.9315984701395527)
  (4.2, 0.9171665732192888)
  (4.21, 0.9012551684123198)
  (4.220000000000001, 0.8835608439179526)
  (4.23, 0.8636673070291221)
  (4.24, 0.840979642438625)
  (4.25, 0.8146012794390542)
  (4.26, 0.783079651389024)
  (4.2700000000000005, 0.7438012742282119)
  (4.28, 0.6912056133474114)
  (4.29, 0.6089267467622664)
  (4.300000000000001, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap5
] coordinates {
  (4.4, 0.0)
  (4.41, 4.049452898020836e-6)
  (4.42, 3.9633866479959063e-5)
  (4.43, 0.00015001642238645453)
  (4.44, 0.0003848255861026075)
  (4.45, 0.0007976249991031842)
  (4.46, 0.0014446220105188892)
  (4.47, 0.0023838145060113797)
  (4.48, 0.0036743652745335163)
  (4.49, 0.005376112783936075)
  (4.5, 0.007549171374677252)
  (4.51, 0.010253593788755337)
  (4.52, 0.0135490791556948)
  (4.53, 0.01749471528361451)
  (4.54, 0.02214874754251335)
  (4.55, 0.02756836880514939)
  (4.56, 0.03380952635083879)
  (4.57, 0.040926742623486834)
  (4.58, 0.048972947430461725)
  (4.59, 0.05799931967158976)
  (4.6, 0.06805513705875514)
  (4.61, 0.07918763256574651)
  (4.62, 0.09144185656123316)
  (4.63, 0.10486054374282087)
  (4.64, 0.11948398411935846)
  (4.65, 0.1353498973907598)
  (4.66, 0.15249331015584142)
  (4.67, 0.17094643544365223)
  (4.68, 0.19073855411586352)
  (4.69, 0.2118958977295537)
  (4.7, 0.23444153248306673)
  (4.71, 0.25839524389400725)
  (4.72, 0.2837734218789866)
  (4.73, 0.31058894592028413)
  (4.74, 0.3388510700158014)
  (4.75, 0.36856530711605073)
  (4.76, 0.3997333127557981)
  (4.77, 0.4323527675886074)
  (4.78, 0.46641725853013616)
  (4.79, 0.5019161582106194)
  (4.8, 0.5388345024286498)
  (4.81, 0.5771528652870355)
  (4.82, 0.6168472316771026)
  (4.83, 0.6578888667601324)
  (4.84, 0.7002441820734966)
  (4.85, 0.7438745978641127)
  (4.86, 0.7887364012227949)
  (4.87, 0.8347805995594162)
  (4.88, 0.8819527689199959)
  (4.89, 0.9301928966022287)
  (4.9, 0.9794352174747986)
  (4.91, 1.0296080433471004)
  (4.92, 1.0806335846686708)
  (4.93, 1.1324277637603033)
  (4.94, 1.1849000186899616)
  (4.95, 1.237953096804277)
  (4.96, 1.2914828368083113)
  (4.97, 1.3453779381497235)
  (4.98, 1.399519716305025)
  (4.99, 1.4537818423813675)
  (5.0, 1.5080300652322707)
  (5.01, 1.562121914033848)
  (5.02, 1.6159063789721373)
  (5.03, 1.6692235673428197)
  (5.04, 1.7219043319507694)
  (5.05, 1.773769868204153)
  (5.06, 1.8246312757086873)
  (5.07, 1.8742890794594589)
  (5.08, 1.9225327048721406)
  (5.09, 1.9691398998556766)
  (5.1, 2.0138760958577024)
  (5.11, 2.0564936982505735)
  (5.12, 2.0967312944898224)
  (5.13, 2.1343127660618073)
  (5.14, 2.1689462872017775)
  (5.15, 2.2003231895165944)
  (5.16, 2.228116666728071)
  (5.17, 2.251980287405377)
  (5.18, 2.271546275279003)
  (5.19, 2.286423505819507)
  (5.2, 2.2961951532112415)
  (5.21, 2.300415902184557)
  (5.22, 2.2986086122139877)
  (5.23, 2.290260284065898)
  (5.24, 2.274817125543973)
  (5.25, 2.2516784366047564)
  (5.26, 2.220188921015307)
  (5.27, 2.1796288612206505)
  (5.28, 2.129201328879502)
  (5.29, 2.0680151815294257)
  (5.3, 1.9950618979636288)
  (5.31, 1.909183103173985)
  (5.32, 1.8090234634828084)
  (5.33, 1.692959483398992)
  (5.34, 1.5589862316946728)
  (5.35, 1.4045250049732745)
  (5.36, 1.2260672978458849)
  (5.37, 1.018431158251848)
  (5.38, 0.7728939767077186)
  (5.39, 0.4706683485094208)
  (5.4, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap6
] coordinates {
  (5.5, 0.0)
  (5.51, 1.1380666180635377e-36)
  (5.52, 2.330768419749756e-30)
  (5.53, 1.1227627487466676e-26)
  (5.54, 4.536934951263491e-24)
  (5.55, 4.713798596817373e-22)
  (5.56, 2.073899302382415e-20)
  (5.57, 5.041859218374425e-19)
  (5.58, 7.93903835915561e-18)
  (5.59, 8.970480802249417e-17)
  (5.6, 7.800352114403427e-16)
  (5.61, 5.4869428360521356e-15)
  (5.62, 3.239372502992374e-14)
  (5.63, 1.650638101085088e-13)
  (5.64, 7.418964550320354e-13)
  (5.65, 2.9923819050509588e-12)
  (5.66, 1.0982546265627188e-11)
  (5.67, 3.709642367306822e-11)
  (5.68, 1.164091131649071e-10)
  (5.69, 3.420476114028605e-10)
  (5.7, 9.473743035848165e-10)
  (5.71, 2.4874712303718688e-9)
  (5.72, 6.221801248845296e-9)
  (5.73, 1.488783827397745e-8)
  (5.74, 3.4206170995334635e-8)
  (5.75, 7.570716347959637e-8)
  (5.76, 1.6186948914353342e-7)
  (5.77, 3.3518367516904364e-7)
  (5.78, 6.736959264592096e-7)
  (5.79, 1.316974834041149e-6)
  (5.8, 2.5084345795712354e-6)
  (5.81, 4.662735449906284e-6)
  (5.82, 8.470790810785898e-6)
  (5.83, 1.505999030066229e-5)
  (5.84, 2.6233866871908272e-5)
  (5.85, 4.482384901129392e-5)
  (5.86, 7.519617150968473e-5)
  (5.87, 0.00012396961440444565)
  (5.88, 0.00020101451725319273)
  (5.89, 0.0003208202990239562)
  (5.9, 0.000504337059542056)
  (5.91, 0.0007814159534198393)
  (5.92, 0.0011939916817980672)
  (5.93, 0.0018001668904647592)
  (5.94, 0.002679370151193026)
  (5.95, 0.003938763549542612)
  (5.96, 0.005721069063235253)
  (5.97, 0.008213960628469224)
  (5.98, 0.01166112628427816)
  (5.99, 0.01637503696818553)
  (6.0, 0.0227513603036076)
  (6.01, 0.03128482436497651)
  (6.02, 0.04258616417231072)
  (6.03, 0.05739957042173479)
  (6.04, 0.07661980600216824)
  (6.05, 0.1013078648210539)
  (6.06, 0.13270372732010943)
  (6.07, 0.17223443106573658)
  (6.08, 0.2215153424293235)
  (6.09, 0.2823422130768607)
  (6.1, 0.3566713666170015)
  (6.11, 0.44658522754979735)
  (6.12, 0.5542404245847579)
  (6.13, 0.6817959266782164)
  (6.14, 0.8313191587484149)
  (6.15, 1.0046688499788106)
  (6.16, 1.2033545399134011)
  (6.17, 1.42837424264623)
  (6.18, 1.6800337632728661)
  (6.19, 1.9577535595747757)
  (6.2, 2.259871791719731)
  (6.21, 2.5834551987738417)
  (6.22, 2.9241325169089674)
  (6.23, 3.275968073985966)
  (6.24, 3.631395646230331)
  (6.25, 3.981234255597307)
  (6.26, 4.31480786147437)
  (6.27, 4.620189344576211)
  (6.28, 4.884585258314302)
  (6.29, 5.094871021952643)
  (6.3, 5.238276130501379)
  (6.31, 5.303205320275845)
  (6.32, 5.28016451416278)
  (6.33, 5.162740268782034)
  (6.34, 4.948559440389306)
  (6.35, 4.640133720081439)
  (6.36, 4.245474323222523)
  (6.37, 3.778349257077191)
  (6.38, 3.2580541224949364)
  (6.39, 2.7085831932496367)
  (6.4, 2.157127037847807)
  (6.41, 1.6318925357645284)
  (6.42, 1.1593456088455325)
  (6.43, 0.7611173432291441)
  (6.44, 0.45098393241757023)
  (6.45, 0.23251028728581488)
  (6.46, 0.09809423641441263)
  (6.47, 0.030184435685424355)
  (6.48, 0.005231457292727744)
  (6.49, 0.00022385869436292145)
  (6.5, 0.0)
};

\addplot+[
  mark = {none},
  very thick, solid, cmap7
] coordinates {
  (6.6, 0.0)
  (6.61, 7.507122664564657e-68)
  (6.62, 3.7667020941032015e-56)
  (6.63, 2.5318111267299745e-49)
  (6.64, 1.7200359380437549e-44)
  (6.65, 9.421051519593204e-41)
  (6.66, 1.0490742073275874e-37)
  (6.67, 3.889796308363498e-35)
  (6.68, 6.44698561448283e-33)
  (6.69, 5.775467727702381e-31)
  (6.7, 3.183752854965566e-29)
  (6.71, 1.1846267725853986e-27)
  (6.72, 3.185439842245949e-26)
  (6.73, 6.5195973731569055e-25)
  (6.74, 1.0573924745902021e-23)
  (6.75, 1.4030921575929693e-22)
  (6.76, 1.5629664680621712e-21)
  (6.77, 1.4926827973602045e-20)
  (6.78, 1.24368138242638e-19)
  (6.79, 9.173020618625014e-19)
  (6.8, 6.0636828251040424e-18)
  (6.81, 3.6303882996099e-17)
  (6.82, 1.986519071733827e-16)
  (6.83, 1.0012877290320574e-15)
  (6.84, 4.680772352125698e-15)
  (6.85, 2.0415897249853264e-14)
  (6.86, 8.352237034304714e-14)
  (6.87, 3.2199513188550413e-13)
  (6.88, 1.174660737082019e-12)
  (6.89, 4.070088185104473e-12)
  (6.9, 1.3439034123347432e-11)
  (6.91, 4.2413551399742405e-11)
  (6.92, 1.2828802855861787e-10)
  (6.93, 3.727980585118243e-10)
  (6.94, 1.0431096109039002e-9)
  (6.95, 2.815987364512808e-9)
  (6.96, 7.348083082087169e-9)
  (6.97, 1.856474319144491e-8)
  (6.98, 4.548228086601546e-8)
  (6.99, 1.0820440750553221e-7)
  (7.0, 2.50298171735363e-7)
  (7.01, 5.636315287635875e-7)
  (7.02, 1.2368898612540852e-6)
  (7.03, 2.647891775477341e-6)
  (7.04, 5.534818552122298e-6)
  (7.05, 1.1306000611128926e-5)
  (7.06, 2.2586869146509294e-5)
  (7.07, 4.416274377381999e-5)
  (7.08, 8.456586823564771e-5)
  (7.09, 0.00015868485074283875)
  (7.1, 0.00029195570749579106)
  (7.11, 0.0005269365815375153)
  (7.12, 0.0009333795891991413)
  (7.13, 0.0016232910617095773)
  (7.14, 0.0027728979049403894)
  (7.15, 0.004653870299314832)
  (7.16, 0.007676511464891236)
  (7.17, 0.012447789417400951)
  (7.18, 0.019846874507843233)
  (7.19, 0.031120024165527237)
  (7.2, 0.04799493942390843)
  (7.21, 0.07281180369539621)
  (7.22, 0.10866383313448551)
  (7.23, 0.1595341658880524)
  (7.24, 0.23040837070302383)
  (7.25, 0.32733320948347794)
  (7.26, 0.4573835067997169)
  (7.27, 0.6284916680028946)
  (7.28, 0.849090849606087)
  (7.29, 1.1275259433260718)
  (7.3, 1.471199650431297)
  (7.31, 1.8854470527398561)
  (7.32, 2.3721732414057843)
  (7.33, 2.928344598177435)
  (7.34, 3.544491675836007)
  (7.35, 4.203452166555833)
  (7.36, 4.879642818888335)
  (7.37, 5.539181107753939)
  (7.38, 6.141159699414375)
  (7.39, 6.640288854171481)
  (7.4, 6.990950261235745)
  (7.41, 7.152451198023355)
  (7.42, 7.094953396242637)
  (7.43, 6.80522757443864)
  (7.44, 6.291131427695926)
  (7.45, 5.583624342056691)
  (7.46, 4.735312848832241)
  (7.47, 3.8150284406037382)
  (7.48, 2.898759500518541)
  (7.49, 2.058264492396913)
  (7.5, 1.3496296919690391)
  (7.51, 0.8045511151997561)
  (7.52, 0.4268663343287593)
  (7.53, 0.19564741245000572)
  (7.54, 0.07414882920810986)
  (7.55, 0.021712378379165412)
  (7.56, 0.004384042575683734)
  (7.57, 0.0004931121238963647)
  (7.58, 1.9135669567948187e-5)
  (7.59, 5.553021267064501e-8)
  (7.6, 0.0)
};

==> figures/subplots/kernel_points_2.tex <==
\addplot+[
  mark = {none},
  very thick, solid, cmap1
] coordinates {
  (0.0, 0.0)
  (0.01, 5.550677207968732e-8)
  (0.02, 1.912951237119128e-5)
  (0.03, 0.0004929823367940944)
  (0.04, 0.004383070420702646)
  (0.05, 0.02170826004714569)
  (0.06, 0.07413670296230872)
  (0.07, 0.19561972863483018)
  (0.08, 0.4268140614008807)
  (0.09, 0.8044660674541794)
  (0.1, 1.3495071884434182)
  (0.11, 2.0581054037616515)
  (0.12, 2.89857100283699)
  (0.13, 3.814823274817849)
  (0.14, 4.735107353431135)
  (0.15, 5.583435826514518)
  (0.16, 6.290975533767979)
  (0.17, 6.805116164987361)
  (0.18, 7.094893295572271)
  (0.19, 7.152443868035548)
  (0.2, 6.990992298270719)
  (0.21, 6.640373066135965)
  (0.22, 6.141276477392223)
  (0.23, 5.539319826638923)
  (0.24, 4.8797930639865035)
  (0.25, 4.203604662935149)
  (0.26, 3.544638874475917)
  (0.27, 2.928480934847544)
  (0.28, 2.372295125009584)
  (0.29, 1.8855526596350334)
  (0.3, 1.4712886036777877)
  (0.31, 1.1275989462784768)
  (0.32, 0.8491493272276314)
  (0.33, 0.628537451326421)
  (0.34, 0.45741857935644525)
  (0.35, 0.3273595211436882)
  (0.36, 0.2304277149363413)
  (0.37, 0.15954811082360382)
  (0.38, 0.10867369434865229)
  (0.39, 0.07281864652892603)
  (0.4, 0.04799959997853381)
  (0.41, 0.031123140224292745)
  (0.42, 0.01984891991576549)
  (0.43, 0.012449107590588428)
  (0.44, 0.007677345471341369)
  (0.45, 0.004654388302665539)
  (0.46, 0.002773213696524393)
  (0.47, 0.0016234799867269822)
  (0.48, 0.0009334904794561517)
  (0.49, 0.0005270004203041085)
  (0.5, 0.0002919917415373101)
  (0.51, 0.0001587047853086386)
  (0.52, 8.457667189831644e-5)
  (0.53, 4.4168476843367073e-5)
  (0.54, 2.2589846376149423e-5)
  (0.55, 1.1307512700909492e-5)
  (0.56, 5.5355691146789845e-6)
  (0.57, 2.6482556195224344e-6)
  (0.58, 1.2370619714962984e-6)
  (0.59, 5.637109016045207e-7)
  (0.6, 2.503338238747164e-7)
  (0.61, 1.0821998807521047e-7)
  (0.62, 4.5488897819864407e-8)
  (0.63, 1.8567470637524808e-8)
  (0.64, 7.349172695436916e-9)
  (0.65, 2.816408619402087e-9)
  (0.66, 1.0432669544622357e-9)
  (0.67, 3.728547332514986e-10)
  (0.68, 1.283076754277213e-10)
  (0.69, 4.242009172139436e-11)
  (0.7, 1.3441119796441084e-11)
  (0.71, 4.070723606397373e-12)
  (0.72, 1.1748451302291166e-12)
  (0.73, 3.2204593005856336e-13)
  (0.74, 8.353560633258193e-14)
  (0.75, 2.041914558015106e-14)
  (0.76, 4.681519702181087e-15)
  (0.77, 1.0014480715696887e-15)
  (0.78, 1.986837949426744e-16)
  (0.79, 3.630972109861184e-17)
  (0.8, 6.064659101475554e-18)
  (0.81, 9.174498291209005e-19)
  (0.82, 1.243881688385636e-19)
  (0.83, 1.4929229752665405e-20)
  (0.84, 1.5632174972860819e-21)
  (0.85, 1.4033168854053488e-22)
  (0.86, 1.0575611836024348e-23)
  (0.87, 6.520632336575183e-25)
  (0.88, 3.1859422588674996e-26)
  (0.89, 1.184812103460483e-27)
  (0.9, 3.184245934602874e-29)
  (0.91, 5.776351060852859e-31)
  (0.92, 6.447956424229388e-33)
  (0.93, 3.89037073745852e-35)
  (0.94, 1.0492253367717374e-37)
  (0.95, 9.422365590501466e-41)
  (0.96, 1.7202655966101187e-44)
  (0.97, 2.5321285560105346e-49)
  (0.98, 3.767128737419213e-56)
  (0.99, 7.50780951836119e-68)
  (1.0, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap2
] coordinates {
  (1.1, 0.0)
  (1.11, 1.101184133815653e-5)
  (1.12, 0.0006868092703380985)
  (1.13, 0.006841457749806506)
  (1.14, 0.03210173579826677)
  (1.15, 0.09957855516468056)
  (1.16, 0.23746921896803566)
  (1.17, 0.4718499970366009)
  (1.18, 0.8196075558576992)
  (1.19, 1.2836622941822105)
  (1.2, 1.8514110923106826)
  (1.21, 2.4962540104567834)
  (1.22, 3.1813977868499252)
  (1.23, 3.864858742664465)
  (1.24, 4.504625896327868)
  (1.25, 5.063170051155577)
  (1.26, 5.510786566400998)
  (1.27, 5.8275576510636835)
  (1.28, 6.003965362161811)
  (1.29, 6.040357371727115)
  (1.3, 5.9455622219189355)
  (1.31, 5.734979785320785)
  (1.32, 5.428452514073478)
  (1.33, 5.048171588637345)
  (1.34, 4.616805316375087)
  (1.35, 4.155967812483051)
  (1.36, 3.685083015620005)
  (1.37, 3.220647700295382)
  (1.38, 2.775859555334985)
  (1.39, 2.3605525318755602)
  (1.4, 1.9813699496226043)
  (1.41, 1.6421038869973201)
  (1.42, 1.344134486225658)
  (1.43, 1.086912398145787)
  (1.44, 0.8684394388910575)
  (1.45, 0.6857148651175962)
  (1.46, 0.5351262285074038)
  (1.47, 0.41277374297501035)
  (1.48, 0.3147250850097648)
  (1.49, 0.237203453686416)
  (1.5, 0.17671566622720603)
  (1.51, 0.13012931910210504)
  (1.52, 0.09470893383365966)
  (1.53, 0.06812087737658573)
  (1.54, 0.04841602480095101)
  (1.55, 0.03399789900514579)
  (1.56, 0.02358260543427435)
  (1.57, 0.01615544910953896)
  (1.58, 0.010927792903277216)
  (1.59, 0.0072965599071067155)
  (1.6, 0.004807831825073855)
  (1.61, 0.0031252548203630146)
  (1.62, 0.002003420519143377)
  (1.63, 0.0012660179303319238)
  (1.64, 0.0007883214933902262)
  (1.65, 0.0004834599725017467)
  (1.66, 0.00029187115484888385)
  (1.67, 0.0001733627647939567)
  (1.68, 0.0001012497782671972)
  (1.69, 5.8106262469353146e-5)
  (1.7, 3.27442322411805e-5)
  (1.71, 1.8104863772258026e-5)
  (1.72, 9.813873730148405e-6)
  (1.73, 5.210438696087693e-6)
  (1.74, 2.706854767066299e-6)
  (1.75, 1.3744888185438193e-6)
  (1.76, 6.813777597763719e-7)
  (1.77, 3.2933748081173986e-7)
  (1.78, 1.549822744488202e-7)
  (1.79, 7.089738270512891e-8)
  (1.8, 3.147283194848905e-8)
  (1.81, 1.3532257975369855e-8)
  (1.82, 5.6236105117891364e-9)
  (1.83, 2.2534598103556583e-9)
  (1.84, 8.684306786630187e-10)
  (1.85, 3.2091946013772897e-10)
  (1.86, 1.1334407258961668e-10)
  (1.87, 3.811749794256618e-11)
  (1.88, 1.2154455201949522e-11)
  (1.89, 3.657094157331411e-12)
  (1.9, 1.0325739505119214e-12)
  (1.91, 2.718397091436798e-13)
  (1.92, 6.623394739371936e-14)
  (1.93, 1.48059777855097e-14)
  (1.94, 3.0054074662851847e-15)
  (1.95, 5.471801027197253e-16)
  (1.96, 8.803556064814913e-17)
  (1.97, 1.2290990045082392e-17)
  (1.98, 1.4558425683576771e-18)
  (1.99, 1.4219140711864904e-19)
  (2.0, 1.1039530828307158e-20)
  (2.01, 6.492155793096311e-22)
  (2.02, 2.7089555899243936e-23)
  (2.03, 7.317926778843856e-25)
  (2.04, 1.1190559590098956e-26)
  (2.05, 7.867034743438656e-29)
  (2.06, 1.7940921579850465e-31)
  (2.07, 6.903733678720191e-35)
  (2.08, 1.0332951842855756e-39)
  (2.09, 5.567547094862992e-48)
  (2.1, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap3
] coordinates {
  (2.2, 0.0)
  (2.21, 0.022356044704381264)
  (2.22, 0.10649103588561323)
  (2.23, 0.25443034685878335)
  (2.24, 0.45800161478846607)
  (2.25, 0.7056316351277697)
  (2.26, 0.9848272639827502)
  (2.27, 1.2833986294801922)
  (2.28, 1.5901081935343053)
  (2.29, 1.8950076362057489)
  (2.3, 2.189589012536365)
  (2.31, 2.466820167421992)
  (2.32, 2.7211067512469014)
  (2.33, 2.9482080400419544)
  (2.34, 3.145124760452583)
  (2.35, 3.3099714202869404)
  (2.36, 3.4418418600437315)
  (2.37, 3.5406741318513184)
  (2.38, 3.607118962218547)
  (2.39, 3.6424147147079893)
  (2.4, 3.6482707824365677)
  (2.41, 3.6267606070784053)
  (2.42, 3.5802249728450923)
  (2.43, 3.5111858137087566)
  (2.44, 3.422270466483225)
  (2.45, 3.3161460769744386)
  (2.46, 3.195463703206983)
  (2.47, 3.062811545092865)
  (2.48, 2.920676653363404)
  (2.49, 2.771414423989564)
  (2.5, 2.6172251612550728)
  (2.51, 2.460136988016937)
  (2.52, 2.301994391394962)
  (2.53, 2.144451712867398)
  (2.54, 1.9889709208260207)
  (2.55, 1.8368230388683304)
  (2.56, 1.6890926426838064)
  (2.57, 1.546684880857022)
  (2.58, 1.4103345190608816)
  (2.59, 1.280616551967178)
  (2.6, 1.1579579719606594)
  (2.61, 1.0426503277622956)
  (2.62, 0.9348627488315308)
  (2.63, 0.8346551525191023)
  (2.64, 0.7419913900665848)
  (2.65, 0.6567521244595085)
  (2.66, 0.5787472676675536)
  (2.67, 0.5077278368340113)
  (2.68, 0.4433971184417776)
  (2.69, 0.3854210563593612)
  (2.7, 0.33343780396715056)
  (2.71, 0.28706640231960107)
  (2.72, 0.24591456557570823)
  (2.73, 0.2095855718104925)
  (2.74, 0.1776842719033996)
  (2.75, 0.14982224159761007)
  (2.76, 0.12562211216011723)
  (2.77, 0.10472112347656477)
  (2.78, 0.08677395002375721)
  (2.79, 0.07145485511660617)
  (2.8, 0.05845923226736125)
  (2.81, 0.047504594566097735)
  (2.82, 0.03833107383460074)
  (2.83, 0.030701491060964738)
  (2.84, 0.02440105842631785)
  (2.85, 0.01923677122095647)
  (2.86, 0.015036545242895886)
  (2.87, 0.011648151999906618)
  (2.88, 0.00893800031288066)
  (2.89, 0.006789808853534787)
  (2.9, 0.005103209845581767)
  (2.91, 0.00379231971067966)
  (2.92, 0.0027843079360349763)
  (2.93, 0.0020179909588396733)
  (2.94, 0.0014424734749693103)
  (2.95, 0.0010158553485413672)
  (2.96, 0.0007040182797310668)
  (2.97, 0.00047950262712545094)
  (2.98, 0.0003204813161429478)
  (2.99, 0.00020983462688411392)
  (3.0, 0.00013432686556186143)
  (3.01, 8.388349809021444e-5)
  (3.02, 5.0965269816811984e-5)
  (3.03, 3.0034152041233072e-5)
  (3.04, 1.710463746079591e-5)
  (3.05, 9.372940355693689e-6)
  (3.06, 4.916024696774226e-6)
  (3.07, 2.4520606815093008e-6)
  (3.08, 1.1538690125933965e-6)
  (3.09, 5.071199710672618e-7)
  (3.1, 2.054750250264462e-7)
  (3.11, 7.54536940543155e-8)
  (3.12, 2.453710885469736e-8)
  (3.13, 6.840593980713712e-9)
  (3.14, 1.5590100797936264e-9)
  (3.15, 2.6982598777824205e-10)
  (3.16, 3.134577062527532e-11)
  (3.17, 1.939162075782281e-12)
  (3.18, 3.7993925686421565e-14)
  (3.19, 4.491202607995046e-17)
  (3.2, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap4
] coordinates {
  (3.3000000000000003, 0.0)
  (3.31, 0.0021083978053842217)
  (3.3200000000000003, 0.008902621728019606)
  (3.33, 0.02048780886055196)
  (3.3400000000000003, 0.036770241135637115)
  (3.35, 0.057581932683835366)
  (3.3600000000000003, 0.08271514156963455)
  (3.37, 0.11193811731362409)
  (3.3800000000000003, 0.14500385717954958)
  (3.39, 0.18165557531364152)
  (3.4000000000000004, 0.22163039563380033)
  (3.41, 0.2646619895701711)
  (3.4200000000000004, 0.3104825420487061)
  (3.43, 0.35882426645304943)
  (3.4400000000000004, 0.4094206037134985)
  (3.45, 0.4620071924336019)
  (3.4600000000000004, 0.5163226682350206)
  (3.47, 0.572109332596084)
  (3.4800000000000004, 0.6291137198681006)
  (3.49, 0.6870870834025921)
  (3.5000000000000004, 0.7457858163931388)
  (3.5100000000000002, 0.8049718192806835)
  (3.5200000000000005, 0.8644128228684765)
  (3.5300000000000002, 0.923882674310167)
  (3.54, 0.9831615916551533)
  (3.5500000000000003, 1.0420363915144648)
  (3.5600000000000005, 1.1003006935493678)
  (3.5700000000000003, 1.1577551048150778)
  (3.58, 1.2142073864648057)
  (3.5900000000000003, 1.269472604900097)
  (3.6, 1.323373269116718)
  (3.6100000000000003, 1.375739455722359)
  (3.62, 1.4264089228793262)
  (3.6300000000000003, 1.4752272142415175)
  (3.64, 1.5220477538022867)
  (3.6500000000000004, 1.566731932442118)
  (3.66, 1.6091491868574797)
  (3.6700000000000004, 1.649177071460995)
  (3.68, 1.6867013237652781)
  (3.6900000000000004, 1.7216159236958175)
  (3.7, 1.753823147220508)
  (3.7100000000000004, 1.7832336146329655)
  (3.72, 1.8097663337826722)
  (3.7300000000000004, 1.833348738505926)
  (3.74, 1.8539167224768625)
  (3.7500000000000004, 1.8714146686666941)
  (3.7600000000000002, 1.885795474571115)
  (3.7700000000000005, 1.8970205733400751)
  (3.7800000000000002, 1.9050599509204154)
  (3.79, 1.9098921592996787)
  (3.8000000000000003, 1.9115043259185853)
  (3.8100000000000005, 1.9098921592996787)
  (3.8200000000000003, 1.9050599509204154)
  (3.83, 1.8970205733400751)
  (3.8400000000000003, 1.885795474571115)
  (3.8500000000000005, 1.8714146686666941)
  (3.8600000000000003, 1.8539167224768625)
  (3.87, 1.833348738505926)
  (3.8800000000000003, 1.8097663337826722)
  (3.89, 1.7832336146329655)
  (3.9000000000000004, 1.753823147220508)
  (3.91, 1.7216159236958175)
  (3.9200000000000004, 1.6867013237652781)
  (3.93, 1.649177071460995)
  (3.9400000000000004, 1.6091491868574797)
  (3.95, 1.566731932442118)
  (3.9600000000000004, 1.5220477538022867)
  (3.97, 1.4752272142415175)
  (3.9800000000000004, 1.4264089228793255)
  (3.99, 1.3757394557223597)
  (4.0, 1.323373269116718)
  (4.01, 1.269472604900097)
  (4.0200000000000005, 1.2142073864648057)
  (4.03, 1.1577551048150778)
  (4.04, 1.1003006935493678)
  (4.050000000000001, 1.0420363915144648)
  (4.0600000000000005, 0.9831615916551533)
  (4.07, 0.923882674310167)
  (4.08, 0.8644128228684762)
  (4.09, 0.8049718192806832)
  (4.1000000000000005, 0.7457858163931385)
  (4.11, 0.6870870834025921)
  (4.12, 0.6291137198681006)
  (4.130000000000001, 0.572109332596084)
  (4.140000000000001, 0.516322668235021)
  (4.15, 0.46200719243360233)
  (4.16, 0.4094206037134985)
  (4.17, 0.35882426645304943)
  (4.180000000000001, 0.3104825420487061)
  (4.19, 0.2646619895701707)
  (4.2, 0.22163039563380013)
  (4.21, 0.18165557531364152)
  (4.220000000000001, 0.14500385717954944)
  (4.23, 0.1119381173136239)
  (4.24, 0.0827151415696347)
  (4.25, 0.057581932683835414)
  (4.26, 0.03677024113563721)
  (4.2700000000000005, 0.020487808860552015)
  (4.28, 0.008902621728019621)
  (4.29, 0.0021083978053842217)
  (4.300000000000001, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap5
] coordinates {
  (4.4, 0.0)
  (4.41, 4.4912026079950775e-17)
  (4.42, 3.799392568642143e-14)
  (4.43, 1.939162075782274e-12)
  (4.44, 3.1345770625275093e-11)
  (4.45, 2.698259877782411e-10)
  (4.46, 1.5590100797936208e-9)
  (4.47, 6.840593980713785e-9)
  (4.48, 2.4537108854697535e-8)
  (4.49, 7.54536940543155e-8)
  (4.5, 2.0547502502644804e-7)
  (4.51, 5.071199710672646e-7)
  (4.52, 1.1538690125933986e-6)
  (4.53, 2.452060681509305e-6)
  (4.54, 4.9160246967742345e-6)
  (4.55, 9.372940355693706e-6)
  (4.56, 1.7104637460795942e-5)
  (4.57, 3.0034152041233127e-5)
  (4.58, 5.096526981681189e-5)
  (4.59, 8.388349809021459e-5)
  (4.6, 0.00013432686556186167)
  (4.61, 0.00020983462688411468)
  (4.62, 0.00032048131614294896)
  (4.63, 0.00047950262712545094)
  (4.64, 0.000704018279731068)
  (4.65, 0.0010158553485413672)
  (4.66, 0.001442473474969313)
  (4.67, 0.002017990958839677)
  (4.68, 0.002784307936034981)
  (4.69, 0.0037923197106796533)
  (4.7, 0.0051032098455817574)
  (4.71, 0.006789808853534775)
  (4.72, 0.008938000312880676)
  (4.73, 0.011648151999906639)
  (4.74, 0.01503654524289594)
  (4.75, 0.01923677122095647)
  (4.76, 0.02440105842631785)
  (4.77, 0.030701491060964738)
  (4.78, 0.03833107383460074)
  (4.79, 0.047504594566097735)
  (4.8, 0.05845923226736125)
  (4.81, 0.07145485511660604)
  (4.82, 0.08677395002375705)
  (4.83, 0.10472112347656477)
  (4.84, 0.12562211216011723)
  (4.85, 0.14982224159761007)
  (4.86, 0.17768427190339994)
  (4.87, 0.2095855718104925)
  (4.88, 0.2459145655757078)
  (4.89, 0.28706640231960157)
  (4.9, 0.33343780396715056)
  (4.91, 0.3854210563593605)
  (4.92, 0.4433971184417768)
  (4.93, 0.5077278368340113)
  (4.94, 0.5787472676675536)
  (4.95, 0.6567521244595085)
  (4.96, 0.7419913900665848)
  (4.97, 0.8346551525191008)
  (4.98, 0.9348627488315291)
  (4.99, 1.0426503277622947)
  (5.0, 1.1579579719606585)
  (5.01, 1.2806165519671768)
  (5.02, 1.4103345190608816)
  (5.03, 1.5466848808570206)
  (5.04, 1.6890926426838064)
  (5.05, 1.8368230388683287)
  (5.06, 1.9889709208260207)
  (5.07, 2.144451712867398)
  (5.08, 2.301994391394962)
  (5.09, 2.460136988016935)
  (5.1, 2.617225161255068)
  (5.11, 2.771414423989559)
  (5.12, 2.9206766533634014)
  (5.13, 3.062811545092865)
  (5.14, 3.19546370320698)
  (5.15, 3.3161460769744355)
  (5.16, 3.422270466483222)
  (5.17, 3.5111858137087566)
  (5.18, 3.5802249728450923)
  (5.19, 3.6267606070784053)
  (5.2, 3.6482707824365646)
  (5.21, 3.642414714707986)
  (5.22, 3.607118962218544)
  (5.23, 3.5406741318513153)
  (5.24, 3.4418418600437284)
  (5.25, 3.3099714202869404)
  (5.26, 3.1451247604525805)
  (5.27, 2.9482080400419544)
  (5.28, 2.7211067512469014)
  (5.29, 2.46682016742199)
  (5.3, 2.1895890125363633)
  (5.31, 1.895007636205747)
  (5.32, 1.590108193534304)
  (5.33, 1.283398629480189)
  (5.34, 0.9848272639827502)
  (5.35, 0.7056316351277704)
  (5.36, 0.45800161478846685)
  (5.37, 0.25443034685878424)
  (5.38, 0.10649103588561341)
  (5.39, 0.022356044704381264)
  (5.4, 0.0)
};

\addplot+[
  mark = {none},
  solid, cmap6
] coordinates {
  (5.5, 0.0)
  (5.51, 5.567547094862992e-48)
  (5.52, 1.0332951842855462e-39)
  (5.53, 6.903733678719797e-35)
  (5.54, 1.7940921579849955e-31)
  (5.55, 7.867034743438209e-29)
  (5.56, 1.1190559590098478e-26)
  (5.57, 7.31792677884396e-25)
  (5.58, 2.7089555899243936e-23)
  (5.59, 6.492155793096311e-22)
  (5.6, 1.1039530828307158e-20)
  (5.61, 1.4219140711865005e-19)
  (5.62, 1.4558425683576667e-18)
  (5.63, 1.2290990045082304e-17)
  (5.64, 8.80355606481485e-17)
  (5.65, 5.471801027197214e-16)
  (5.66, 3.0054074662851417e-15)
  (5.67, 1.4805977785509594e-14)
  (5.68, 6.623394739371842e-14)
  (5.69, 2.718397091436798e-13)
  (5.7, 1.0325739505119286e-12)
  (5.71, 3.657094157331411e-12)
  (5.72, 1.2154455201949522e-11)
  (5.73, 3.811749794256618e-11)
  (5.74, 1.1334407258961587e-10)
  (5.75, 3.209194601377267e-10)
  (5.76, 8.684306786630126e-10)
  (5.77, 2.253459810355642e-9)
  (5.78, 5.623610511789097e-9)
  (5.79, 1.3532257975369759e-8)
  (5.8, 3.147283194848882e-8)
  (5.81, 7.08973827051279e-8)
  (5.82, 1.549822744488202e-7)
  (5.83, 3.2933748081173986e-7)
  (5.84, 6.813777597763768e-7)
  (5.85, 1.3744888185438142e-6)
  (5.86, 2.7068547670662894e-6)
  (5.87, 5.210438696087675e-6)
  (5.88, 9.81387373014837e-6)
  (5.89, 1.8104863772257897e-5)
  (5.9, 3.274423224118038e-5)
  (5.91, 5.810626246935273e-5)
  (5.92, 0.00010124977826719646)
  (5.93, 0.0001733627647939561)
  (5.94, 0.0002918711548488828)
  (5.95, 0.0004834599725017467)
  (5.96, 0.0007883214933902262)
  (5.97, 0.001266017930331915)
  (5.98, 0.00200342051914337)
  (5.99, 0.0031252548203630033)
  (6.0, 0.004807831825073821)
  (6.01, 0.0072965599071066894)
  (6.02, 0.010927792903277138)
  (6.03, 0.016155449109538905)
  (6.04, 0.02358260543427435)
  (6.05, 0.033997899005145674)
  (6.06, 0.04841602480095101)
  (6.07, 0.06812087737658525)
  (6.08, 0.094708933833659)
  (6.09, 0.1301293191021046)
  (6.1, 0.1767156662272054)
  (6.11, 0.23720345368641513)
  (6.12, 0.3147250850097637)
  (6.13, 0.4127737429750089)
  (6.14, 0.5351262285074038)
  (6.15, 0.6857148651175962)
  (6.16, 0.8684394388910543)
  (6.17, 1.086912398145787)
  (6.18, 1.344134486225653)
  (6.19, 1.6421038869973144)
  (6.2, 1.9813699496225972)
  (6.21, 2.360552531875552)
  (6.22, 2.775859555334985)
  (6.23, 3.220647700295359)
  (6.24, 3.6850830156199788)
  (6.25, 4.155967812483036)
  (6.26, 4.61680531637507)
  (6.27, 5.048171588637327)
  (6.28, 5.428452514073478)
  (6.29, 5.734979785320766)
  (6.3, 5.9455622219189355)
  (6.31, 6.040357371727094)
  (6.32, 6.003965362161768)
  (6.33, 5.827557651063662)
  (6.34, 5.510786566400978)
  (6.35, 5.063170051155577)
  (6.36, 4.504625896327852)
  (6.37, 3.864858742664451)
  (6.38, 3.1813977868499137)
  (6.39, 2.4962540104567745)
  (6.4, 1.851411092310676)
  (6.41, 1.2836622941822105)
  (6.42, 0.8196075558576963)
  (6.43, 0.4718499970365976)
  (6.44, 0.23746921896803566)
  (6.45, 0.09957855516468056)
  (6.46, 0.03210173579826688)
  (6.47, 0.006841457749806531)
  (6.48, 0.0006868092703381009)
  (6.49, 1.1011841338156453e-5)
  (6.5, 0.0)
};

\addplot+[
  mark = {none},
  very thick, solid, cmap7
] coordinates {
  (6.6, 0.0)
  (6.61, 7.50780951836119e-68)
  (6.62, 3.767128737419106e-56)
  (6.63, 2.5321285560104624e-49)
  (6.64, 1.7202655966100455e-44)
  (6.65, 9.422365590501064e-41)
  (6.66, 1.0492253367716927e-37)
  (6.67, 3.890370737458686e-35)
  (6.68, 6.447956424229479e-33)
  (6.69, 5.776351060852859e-31)
  (6.7, 3.1842459346029643e-29)
  (6.71, 1.1848121034605168e-27)
  (6.72, 3.1859422588674996e-26)
  (6.73, 6.520632336575183e-25)
  (6.74, 1.0575611836024348e-23)
  (6.75, 1.4033168854053488e-22)
  (6.76, 1.5632174972860597e-21)
  (6.77, 1.4929229752665405e-20)
  (6.78, 1.2438816883856184e-19)
  (6.79, 9.174498291209136e-19)
  (6.8, 6.064659101475554e-18)
  (6.81, 3.63097210986121e-17)
  (6.82, 1.9868379494267724e-16)
  (6.83, 1.0014480715696887e-15)
  (6.84, 4.681519702181087e-15)
  (6.85, 2.041914558015106e-14)
  (6.86, 8.353560633258193e-14)
  (6.87, 3.2204593005856336e-13)
  (6.88, 1.1748451302291166e-12)
  (6.89, 4.070723606397345e-12)
  (6.9, 1.3441119796440989e-11)
  (6.91, 4.2420091721394056e-11)
  (6.92, 1.283076754277222e-10)
  (6.93, 3.7285473325150124e-10)
  (6.94, 1.0432669544622503e-9)
  (6.95, 2.816408619402087e-9)
  (6.96, 7.349172695436916e-9)
  (6.97, 1.8567470637524808e-8)
  (6.98, 4.5488897819864407e-8)
  (6.99, 1.0821998807521047e-7)
  (7.0, 2.503338238747164e-7)
  (7.01, 5.637109016045207e-7)
  (7.02, 1.2370619714962895e-6)
  (7.03, 2.6482556195224154e-6)
  (7.04, 5.5355691146789845e-6)
  (7.05, 1.1307512700909572e-5)
  (7.06, 2.2589846376149423e-5)
  (7.07, 4.4168476843367073e-5)
  (7.08, 8.457667189831644e-5)
  (7.09, 0.0001587047853086386)
  (7.1, 0.0002919917415373101)
  (7.11, 0.0005270004203041085)
  (7.12, 0.0009334904794561517)
  (7.13, 0.0016234799867269822)
  (7.14, 0.002773213696524403)
  (7.15, 0.004654388302665539)
  (7.16, 0.007677345471341396)
  (7.17, 0.012449107590588428)
  (7.18, 0.019848919915765418)
  (7.19, 0.031123140224292523)
  (7.2, 0.04799959997853381)
  (7.21, 0.07281864652892603)
  (7.22, 0.10867369434865229)
  (7.23, 0.15954811082360382)
  (7.24, 0.2304277149363413)
  (7.25, 0.3273595211436882)
  (7.26, 0.45741857935644364)
  (7.27, 0.6285374513264232)
  (7.28, 0.8491493272276314)
  (7.29, 1.1275989462784728)
  (7.3, 1.471288603677777)
  (7.31, 1.8855526596350267)
  (7.32, 2.372295125009584)
  (7.33, 2.928480934847544)
  (7.34, 3.544638874475917)
  (7.35, 4.203604662935149)
  (7.36, 4.8797930639865035)
  (7.37, 5.539319826638923)
  (7.38, 6.141276477392223)
  (7.39, 6.640373066135965)
  (7.4, 6.990992298270719)
  (7.41, 7.152443868035548)
  (7.42, 7.094893295572247)
  (7.43, 6.805116164987361)
  (7.44, 6.290975533768001)
  (7.45, 5.583435826514518)
  (7.46, 4.735107353431135)
  (7.47, 3.814823274817849)
  (7.48, 2.89857100283699)
  (7.49, 2.058105403761644)
  (7.5, 1.3495071884434182)
  (7.51, 0.8044660674541794)
  (7.52, 0.4268140614008792)
  (7.53, 0.1956197286348295)
  (7.54, 0.07413670296230898)
  (7.55, 0.021708260047145843)
  (7.56, 0.004383070420702661)
  (7.57, 0.0004929823367940944)
  (7.58, 1.9129512371191416e-5)
  (7.59, 5.550677207968732e-8)
  (7.6, 0.0)
};
